QuTI! Quantifying Text-Image Consistency in Multimodal Documents

The World Wide Web and social media platforms have become popular sources for news and information. Typically, multimodal information, e.g., image and text is used to convey information more effectively and to attract attention. While in most cases image content is decorative or depicts additional information, it has also been leveraged to spread misinformation and rumors in recent years. In this paper, we present a Web-based demo application that automatically quantifies the cross-modal relations of entities (persons, locations, and events) in image and text. The applications are manifold. For example, the system can help users to explore multimodal articles more efficiently, or can assist human assessors and fact-checking efforts in the verification of the credibility of news stories, tweets, or other multimodal documents.

==> tab_results.tex <==
\renewcommand{\b}{\textbf}
\begin{table}[t]
% \caption{AUC, FRP, AP-clean and AP-tampered at different recall levels of the \textit{TamperedNews~(Top-50\%)} dataset for different entity testsets~(notations according Section~\ref{sec:tampering}.)}
\caption{Results for document verification~(DV) and collection retrieval for the \textit{TamperedNews~(Top-50\%)} dataset for different entity test sets.}
\label{tab:cms_results_tamperednews}
\fontsize{8}{8}\selectfont
\setlength\tabcolsep{4pt}
\renewcommand{\arraystretch}{1.4}
\centering
    \begin{tabularx}{\linewidth}{X | c | c | c c c | c c c}

        \toprule
        
        % \multirow{3}{*}{\b{Test set ($|\set{D}|$)}} & \b{DV} & \multicolumn{7}{c}{\b{Collection Retrieval}} \\
        \multirow{3}{*}{\b{Test set}} & \b{DV} & \multicolumn{7}{c}{\b{Collection Retrieval}} \\
        & \multirow{2}{*}{\b{VA}} & \multirow{2}{*}{\b{AUC}} & \multicolumn{3}{c|}{\b{AP-clean@}} & \multicolumn{3}{c}{\b{AP-tampered@}}  \\
        & & & 25\%     & 50\%    & 100\%     & 25\%   & 50\%    & 100\%  \\
        
        \midrule
        % \b{Persons} (\num{15323})               &&&&&&&&\\
        % \b{Persons}                             & \multicolumn{8}{c}{\num{15323} documents}\\
        \multicolumn{9}{c}{\b{Persons} (\num{16848} documents)}\\
        \midrule
        Random                             & 0.94 & 0.95 & 96.08 & 95.45 & 92.64 & 100.0 & 100.0 & 96.16 \\
        PsC                                & 0.93 & 0.94 & 95.53 & 94.67 & 91.68 & 100.0 & 100.0 & 95.61 \\
        PsG                                & 0.94 & 0.95 & 95.77 & 95.07 & 92.27 & 100.0 & 100.0 & 96.00 \\
        PsCG                               & 0.93 & 0.94 & 95.04 & 94.70 & 91.70 & 100.0 & 100.0 & 95.56 \\
        
        \midrule
        
        % \b{Locations} (\num{30217})             &&&&&&&&\\
        % \b{Locations}                           & \multicolumn{8}{c}{}\\
        % \textbullet$\,$\b{Outdoor} (\num{12780})&&&&&&&&\\
        % \midrule
        % \textbullet$\,$\b{Outdoor}              & \multicolumn{7}{c}{\num{12780} documents}\\
        \multicolumn{9}{c}{\b{Locations - Outdoor} (\num{14113} documents)}\\
        \midrule
        Random                             & 0.88 & 0.85 & 92.57 & 88.02 & 81.71 & 100.0 & 100.0 & 88.82 \\ 
        GCD$_{750}^{2500}$                 & 0.86 & 0.81 & 88.04 & 83.65 & 77.25 & 100.0 & 100.0 & 85.45 \\ 
        GCD$_{200}^{750}$                  & 0.79 & 0.74 & 82.85 & 76.96 & 70.56 & 100.0 & 96.98 & 79.38 \\ 
        GCD$_{25}^{200}$                   & 0.77 & 0.72 & 80.50 & 74.23 & 68.30 & 100.0 & 95.19 & 77.42 \\

        % \textbullet$\,$\b{Indoor} (\num{17437}) &&&&&&&&\\
        \midrule
        % \textbullet$\,$\b{Indoor}               & \multicolumn{8}{c}{\num{17437} documents}\\
        \multicolumn{9}{c}{\b{Locations - Indoor} (\num{19129} documents)}\\
        \midrule
        Random                             & 0.74 & 0.72 & 68.47 & 66.53 & 65.34 & 100.0 & 99.01 & 79.62 \\
        GCD$_{750}^{2500}$                 & 0.73 & 0.70 & 63.62 & 62.86 & 62.72 & 100.0 & 97.57 & 77.80 \\
        GCD$_{200}^{750}$                  & 0.74 & 0.71 & 66.93 & 65.10 & 63.97 & 100.0 & 97.70 & 78.14 \\
        GCD$_{25}^{200}$                   & 0.69 & 0.68 & 55.99 & 57.74 & 59.48 & 100.0 & 95.97 & 76.04 \\
        
        \midrule
        
        % \b{Events} (\num{7554})                &&&&&&&&\\
        % \b{Events}                              & \multicolumn{8}{c}{\num{7554} documents}\\
        \multicolumn{9}{c}{\b{Events} (\num{7734} documents)}\\
        \midrule
        Random                             & 0.92 & 0.91 & 92.20 & 91.26 & 87.61 & 100.0 & 100.0 & 93.66 \\
        EsP                                & 0.75 & 0.71 & 70.72 & 67.30 & 64.92 & 100.0 & 96.72 & 77.68 \\
        
        % \midrule
        % \b{Context} (\num{36217})              &&&&&&&&\\
        % \b{Context}                             & \multicolumn{8}{c}{\num{36217} documents}\\
        % \multicolumn{9}{c}{\b{Context} (\num{36217} documents)}\\
        % \midrule
        % Random                             & 0.81 & 0.80 & 88.95 & 83.03 & 76.32 & 100.0 & 100.0 & 84.79 \\
        % top-$25\%$                         & 0.78 & 0.77 & 83.52 & 78.12 & 72.43 & 100.0 & 99.70 & 82.25 \\
        % top-$10\%$                         & 0.76 & 0.74 & 77.76 & 73.21 & 68.78 & 100.0 & 98.33 & 79.84 \\
        % top-$5\%$                          & 0.74 & 0.71 & 74.31 & 69.89 & 66.22 & 100.0 & 96.84 & 77.92 \\
        
        \bottomrule
        
    \end{tabularx}
\end{table}
